Matching $\leq$ Hybrid $\leq$ Difference in Differences

Since LaLonde's (1986) seminal paper, there has been ongoing interest in estimating treatment effects using pre- and post-intervention data. Scholars have traditionally used experimental benchmarks to evaluate the accuracy of alternative econometric methods, including Matching, Difference-in-Differences (DID), and their hybrid forms (e.g., Heckman et al., 1998b; Dehejia and Wahba, 2002; Smith and Todd, 2005). We revisit these methodologies in the evaluation of job training and educational programs using four datasets (LaLonde, 1986; Heckman et al., 1998a; Smith and Todd, 2005; Chetty et al., 2014a; Athey et al., 2020), and show that the inequality relationship, Matching $\leq$ Hybrid $\leq$ DID, appears as a consistent norm, rather than a mere coincidence. We provide a formal theoretical justification for this puzzling phenomenon under plausible conditions such as negative selection, by generalizing the classical bracketing (Angrist and Pischke, 2009, Section 5). Consequently, when treatments are expected to be non-negative, DID tends to provide optimistic estimates, while Matching offers more conservative ones.

==> preambles.tex <==
\usepackage{apalike}\usepackage{url}\usepackage{hyperref}\usepackage{cite}
\hypersetup{
  colorlinks=true,
  linkcolor=blue,
  filecolor=magenta,      
  urlcolor=cyan,
  pdftitle={Overleaf Example},
  pdfpagemode=FullScreen,
}\urlstyle{same}
\usepackage[utf8]{inputenc}\usepackage{enumerate}\usepackage{amsmath}\usepackage{amssymb}\usepackage{amsthm}\usepackage{graphicx}\usepackage[dvipsnames]{xcolor}\usepackage{tikz}\usepackage{bm}\usepackage{proof}\usepackage{amsfonts}\usepackage{tcolorbox}\usepackage{ascmac}\usepackage{fancybox}
\usepackage[all]{xy}\usepackage{varwidth}\usepackage{etoolbox}\usepackage{siunitx}\usepackage{physics}
\AtBeginDocument{\RenewCommandCopy\qty\SI}  %% told to add this by compiler 7/27/2023
\hypersetup{
    colorlinks,
    citecolor=black,
    filecolor=black,
    linkcolor=black,
    urlcolor=black
}
\usepackage[edges]{forest}
\usepackage{tree}
\newtheorem{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{proposition}{Proposition}[section]
\newtheorem{corollary}{Corollary}[section]
\newtheorem{notation}{Notation}[section]
\newtheorem{lemma}{Lemma}[section]
\newtheorem{assumption}{Assumption}[section]
\newtheorem{innercustomthm}{Condition}
\newtheorem{algorithm}{Algorithm}[section]

\theoremstyle{definition}
\AtEndEnvironment{remark}{\qed}
\newtheorem{remark}{Remark}[section]
\newtheorem{scrap}{Scrap}[section]

\newenvironment{customthm}[1]
  {\renewcommand\theinnercustomthm{#1}\innercustomthm}
  {\endinnercustomthm}

\newcommand{\koko}{{\color{yellow}koko}}
\newcommand{\todo}{{\color{red}todo}}
\newcommand{\que}{{\color{green}queue}}
\newcommand{\yp}[1]{\textcolor{blue}{Park: #1}}
\newcommand{\pending}{{\color{orange}pending}}

%%% added by Hirofumi Shiba 10/27/2022
\newcommand{\sub}{\subset}
\AtBeginDocument{\RenewCommandCopy\qty\SI} 
\newcommand{\mathrf}[1]{\mathrm#1}

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}
\DeclareMathOperator*{\esssup}{ess\,sup}

%%% useful shorthand for frequently occurring characters
\newcommand{\X}{\mathcal{X}}\newcommand{\V}{\mathcal{V}}
\newcommand{\F}{\mathfrak{F}}\newcommand{\Om}{\Omega}\newcommand{\om}{\omega}\newcommand{\R}{\mathbb{R}}\renewcommand{\P}{\mathbb{P}}
\newcommand{\ifquad}{\text{if}\quad}\newcommand{\al}{\alpha}
\newcommand{\Sel}{\mathrm{Sel}}\newcommand{\as}{\text{a.s.}}

%%% useful commands for parentheses
\renewcommand{\abs}[1]{\lvert#1\rvert}\newcommand{\Abs}[1]{\left|#1\right|}\newcommand{\ABs}[1]{\biggl|#1\biggr|}\renewcommand{\norm}[1]{\|#1\|}\newcommand{\Norm}[1]{\left\|#1\right\|}\newcommand{\NOrm}[1]{\biggl\|#1\biggr\|}\newcommand{\Brace}[1]{\left\{#1\right\}}\newcommand{\BRace}[1]{\biggl\{#1\biggr\}}\newcommand{\paren}[1]{\left(#1\right)}\newcommand{\Paren}[1]{\biggr(#1\biggl)}\newcommand{\bracket}[1]{\langle#1\rangle}\newcommand{\brac}[1]{\langle#1\rangle}\newcommand{\Bracket}[1]{\left\langle#1\right\rangle}\newcommand{\Brac}[1]{\left\langle#1\right\rangle}\newcommand{\Square}[1]{\left[#1\right]}\newcommand{\SQuare}[1]{\biggl[#1\biggr]}
\newcommand{\ov}[1]{\overline{#1}}\newcommand{\un}[1]{\underline{#1}}\newcommand{\wt}[1]{\widetilde{#1}}\newcommand{\wh}[1]{\widehat{#1}}
\newcommand{\pp}[2]{\frac{\partial #1}{\partial #2}}\newcommand{\ppp}[3]{\frac{\partial #1}{\partial #2\partial #3}}\renewcommand{\dd}[2]{\frac{d #1}{d #2}}
\newcommand{\floor}[1]{\lfloor#1\rfloor}\newcommand{\Floor}[1]{\left\lfloor#1\right\rfloor}\newcommand{\ceil}[1]{\lceil#1\rceil}
\newcommand{\ocinterval}[1]{(#1]}\newcommand{\cointerval}[1]{[#1)}\newcommand{\COinterval}[1]{\left[#1\right)}
